Merging Position and Orientation Motion Primitives

In this paper, we focus on generating complex robotic trajectories by merging sequential motion primitives. A robotic trajectory is a time series of positions and orientations ending at a desired target. Hence, we first discuss the generation of converging pose trajectories via dynamical systems, providing a rigorous stability analysis. Then, we present approaches to merge motion primitives which represent both the position and the orientation part of the motion. Developed approaches preserve the shape of each learned movement and allow for continuous transitions among succeeding motion primitives. Presented methodologies are theoretically described and experimentally evaluated, showing that it is possible to generate a smooth pose trajectory out of multiple motion primitives.

==> sections/Proposed_Approach_logarithm.tex <==
\section{Coupled Dynamic Movement Primitives}\label{sec:c_dmp}

\subsection{Formulation}
\begin{figure}[t]
\centering
\includegraphics[width=0.8\columnwidth]{img/coupled_dmp.pdf}
\caption{Overview of the coupled DMP approach.}
\end{figure}

\begin{itemize}
\item Clock signal
\begin{equation}
\dot{s} = -\gamma s
\end{equation}
\item Right hand position
\begin{subequations}
\small
\begin{align}
\dot{\bfp}_r &= \bfv_r \label{eq:dmp_right1}\\
\dot{\bfv}_r &= \bfK\left[(\bfg^p_r - \bfp_r) - \bfd^{p,0}_r + \bff^p_r(s)\right] -\bfD\bfv_r \textcolor{dark_green}{ + \bff^p_{r,l}}
\label{eq:dmp_right2}
\end{align}
\normalsize
\end{subequations}
%
\item Left hand position
\begin{subequations}
\small
\begin{align}
\dot{\bfp}_l &= \bfv_l \label{eq:dmp_left1}\\
\dot{\bfv}_l &= \bfK\left[(\bfg^p_l - \bfp_l) - \bfd^{p,0}_l + \bff^p_l(s)\right] -\bfD\bfv_l \textcolor{blue}{ + \bff^p_{l,r}}
\label{eq:dmp_left2}
\end{align}
\normalsize
\end{subequations}
%
\item Relative position
\begin{subequations}
\small
\begin{align}
\dot{\bfp}_{rel} &= \bfv_{rel} \label{eq:dmp_relative1}\\
\dot{\bfv}_{rel} &= \bfK\left[(\bfg^p_{rel} - \bfp_{rel}) - \bfd^{p,0}_{rel} + \bff^p_{rel}(s)\right] -\bfD\bfv_{rel} \label{eq:dmp_relative2}
\end{align}
\normalsize
\end{subequations}
\end{itemize}
where $\bfd^{p,0}_r = (\bfg^p_r-\bfp_{0,r})s$, $\bfd^{p,0}_l = (\bfg^p_l-\bfp_{0,l})s$, and $\bfd^{p,0}_{rel} = (\bfg^p_{rel}-\bfp_{0,rel})s$. The nonlinear forcing terms $\bff^{p}_{i},\,i=r,l,rel$ in \eqref{eq:dmp_right2}, \eqref{eq:dmp_left2}, and \eqref{eq:dmp_relative2} are defined as:
\begin{equation}
\small
\begin{split}
\bff^{p}_{i} = \frac{\sum_{g=1}^{G}\bfw_{g}^{i}\psi_{g}^{i}(s)}{\sum_{g=1}^{G}\psi_{g}^{i}(s)}s,\quad \psi_{g}^{i}(s) = \exp\left(-h^{i}(s-c_{g}^{i})^2\right) \label{eq:force_term}
\end{split}
\normalsize
\end{equation}
Given $h^{i}$ and $c_{g}^{i}$, the parameters $\bfw_{g}^{i}$ are learned from demonstration using weighted least square \cite{DMP}. The green and blue terms in \eqref{eq:dmp_right2} and \eqref{eq:dmp_left2} respectively represent the synchronization forces, computed as:
\begin{subequations}
\small
\begin{align}
\bff^p_{r,l} &= \bfK_f(\bfp_{rel} - (\bfp_r - \bfp_l)) + \bfD_f(\bfv_{rel} - (\bfv_r - \bfv_l)),\label{eq:synchro_force1}\\
\bff^p_{l,r} &= -\bff^p_{r,l}. \label{eq:synchro_force2}
\end{align}
\normalsize
\end{subequations}
\textcolor{red}{Say about force, errors etc.}

Orientation is represented via unit quaternion $\bfq = [\eta, \bfepsilon\tr]\tr$ (no singularities, ...). Cooperative DMP for the orientation are:
%\begin{itemize}
%\item Right hand orientation
\begin{subequations}
\small
\begin{align}
\dot{\bfq}_r &= \frac{1}{2}\tilde{\bfomega}_r \ast \bfq_r  \label{eq:dmp_ori_right1}\\
\dot{\bfomega}_r &= \bfK\left[2\log(\bfg^q_r \ast \overline{\bfq}_r) - \bfd^{q,0}_r + \bff^q_r(s)\right] -\bfD\bfomega_r  \textcolor{dark_green}{ + \bff^q_{r,l}}
\label{eq:dmp_ori_right2}\\
%\end{align}
%\normalsize
%\end{subequations}
%
%\item Left hand orientation
%\begin{subequations}
%\small
%\begin{align}
\dot{\bfq}_l &= \frac{1}{2}\tilde{\bfomega}_l \ast \bfq_l \label{eq:dmp_ori_left1}\\
\dot{\bfomega}_l &= \bfK\left[2\log(\bfg^q_l \ast \overline{\bfq}_l) - \bfd^{q,0}_l + \bff^q_l(s)\right] -\bfD\bfomega_l {\color{blue} + \bff^q_{l,r}}
\label{eq:dmp_ori_left2}\\
%\end{align}
%\normalsize
%\end{subequations}
%
%\item Relative orientation
%\begin{subequations}
%\small
%\begin{align}
\dot{\bfq}_{rel} &= \frac{1}{2}\tilde{\bfomega}_{rel} \ast \bfq_{rel}  \label{eq:dmp_ori_relative1}\\
\dot{\bfomega}_{rel} &= \bfK\left[2\log(\bfg^q_{rel} \ast \overline{\bfq}_{rel}) - \bfd^{q,0}_{rel} + \bff^q_{rel}(s)\right] -\bfD\bfomega_{rel}\label{eq:dmp_ori_relative2}
\end{align}
\normalsize
\end{subequations}
%\end{itemize}
where $\bfq_1 \ast \bfq_2$ indicates the quaternion product. Note that the angular velocities quaternions $\tilde{\bfomega}_r$, $\tilde{\bfomega}_l$, and $\tilde{\bfomega}_{rel}$ in \eqref{eq:dmp_ori_right1}, \eqref{eq:dmp_ori_left1}, and \eqref{eq:dmp_ori_relative1} are quaternions with zero scalar part and the angular velocity as scalar part, e.g. $\tilde{\bfomega}_r = [0, \bfomega_r\tr]\tr$. The nonlinear forcing terms $\bff^{q}_{i},\,i=r,l,rel$ in \eqref{eq:dmp_ori_right2}, \eqref{eq:dmp_ori_left2}, and \eqref{eq:dmp_ori_relative2} are defined as in \eqref{eq:force_term} and learned from demonstration.
The green and blue terms in \eqref{eq:dmp_ori_right2} and \eqref{eq:dmp_ori_left2} respectively represent the synchronization forces, computed as
\begin{subequations}
\small
\begin{align}
\bff^q_{r,l} &= \bfK_f 2 \log{(\bfq_{rel} \ast (\overline{\bfq_r\ast\overline{\bfq}_l}) )} + \bfD_f(\bfomega_{rel} - (\bfomega_r - \bfomega_l))\label{eq:synchro_force_rot1}\\
\bff^q_{l,r} &= -\bff^q_{r,l} \label{eq:synchro_force_rot2}
\end{align}
\normalsize
\end{subequations}
\textcolor{red}{Say about force, errors etc.}
\textcolor{blue}{the positive definite gain matrices $\bfK$ and $\bfD$ can change in each equation. We keep the same symbol to simplify the notation.}

\subsection{Stability analysis}
DMP are proved to be globally asymptotically stable \cite{DMP}, guaranteeing the convergence towards a specified target. We investigate the stability of Coupled DMP using Lyapunov theory \cite{Slotine91}. Note that in C-DMPs the position---\eqref{eq:dmp_right1}--\eqref{eq:dmp_relative2} with coupling forces \eqref{eq:synchro_force1}, \eqref{eq:synchro_force2}---is completely decoupled from the orientation---\eqref{eq:dmp_ori_right1}--\eqref{eq:dmp_ori_relative2} with coupling forces \eqref{eq:synchro_force_rot1}, \eqref{eq:synchro_force_rot2}---and their stability can be analized separately. 

Let us first focus on the position, i.e. on the stability of the system of differential equations \eqref{eq:dmp_right1}--\eqref{eq:dmp_relative2} with coupling forces defined as in \eqref{eq:synchro_force1}, \eqref{eq:synchro_force2}. First, we notice that the relative DMP in \eqref{eq:dmp_relative1}, \eqref{eq:dmp_relative2} is  decoupled from the other differential equations, and that the terms $\bff^{p}_{rel}(s)$ and $\bfd^{p,0}_{rel}$ are bounded and vanish for $t\rightarrow+\infty$. This implies that the relative DMP is stable ($\bfp_{rel}\rightarrow\bfg^{p}_{rel}$ and $\bfv_{rel}\rightarrow\bfzero$) if the gain matrices $\bfK$ and $\bfD$ are positive definite. Given this, and considering that the nonlinear terms $\bff^{p}_{r}(s)$ and $\bff^{p}_{l}(s)$ are bounded and vanish for $t\rightarrow+\infty$, we can conclude the stability of C-DMPs by analyzing the asymptotic behavior of \eqref{eq:dmp_right1}--\eqref{eq:dmp_left2}. For $t\rightarrow+\infty$, we can rewrite \eqref{eq:synchro_force1}, \eqref{eq:synchro_force2}  as:
\begin{subequations}
\small
\begin{align}
\bff^p_{r,l} &= \bfK_f(\bfg^{p}_{rel} - (\bfp_r - \bfp_l)) - \bfD_f(\bfv_r - \bfv_l)\label{eq:synchro_force1_as}\\
\bff^p_{l,r} &= -\bff^p_{r,l} = -\bfK_f(\bfg^{p}_{rel} - (\bfp_r - \bfp_l)) + \bfD_f(\bfv_r - \bfv_l) \label{eq:synchro_force2_as}
\end{align}
\normalsize
\end{subequations}
and \eqref{eq:dmp_right1}--\eqref{eq:dmp_left2} as:
\begin{subequations}
\small
\begin{align}
\dot{\bfp}_r &= \bfv_r \label{eq:dmp_right1_as}\\
\dot{\bfv}_r &= \bfK(\bfg^p_r - \bfp_r)-\bfD\bfv_r +\bfK_f(\bfg^{p}_{rel} - (\bfp_r - \bfp_l)) - \bfD_f(\bfv_r - \bfv_l)\label{eq:dmp_right2_as}\\
\dot{\bfp}_l &= \bfv_l \label{eq:dmp_left1_as}\\
\dot{\bfv}_l &= \bfK(\bfg^p_l - \bfp_l) -\bfD\bfv_l -\bfK_f(\bfg^{p}_{rel} - (\bfp_r - \bfp_l)) + \bfD_f(\bfv_r - \bfv_l)\label{eq:dmp_left2_as}
\end{align}
\end{subequations}
\normalsize
In order to prove the stability of \eqref{eq:dmp_right1_as}--\eqref{eq:dmp_left2_as}, we consider the candidate Lyapunov function:
\begin{equation}
\small
\begin{split}
V^p(\bfx^p) &= \frac{1}{2}(\bfg^p_r-\bfp_r)\tr\bfK(\bfg^p_r-\bfp_r) +
    \frac{1}{2}(\bfg^p_l-\bfp_l)\tr\bfK(\bfg^p_l-\bfp_l) \\
    &\quad+\frac{1}{2}(\bfg^{p}_{rel}-\bfp_{e})\tr\bfK_f(\bfg^{p}_{rel}-\bfp_{e}) +
    \frac{1}{2}\bfv_r\tr\bfv_r + \frac{1}{2}\bfv_l\tr\bfv_l\label{eq:lyapunov_fun}
\end{split}
\normalsize
\end{equation}
where $\bfp_{e} = \bfp_r - \bfp_l$ and the state is defined as $\bfx^p = [\bfp_r\tr,\, \bfp_l\tr,\, \bfv_r\tr,\, \bfv_l\tr]\tr\in\mathbb{R}^{12}$.  The candidate Lyapunov function in \eqref{eq:lyapunov_fun} is positive definite if $\bfK$, $\bfD$, $\bfK_f$, and $\bfD_f$ are positive definite matrices, and it vanishes only at the equilibrium point $\hat{\bfx}^p =[{\bfg^{p}_{r}}\tr,\, {\bfg^{p}_{l}}\tr,\, \bfzero\tr,\, \bfzero\tr]\tr$ if and only if $\bfg^{p}_{r}-\bfg^{p}_{l} = \bfg^{p}_{rel}$. To show that $V^p(\bfx^p)$ is a proper Lyapunov function, which implies that the system \eqref{eq:dmp_right1_as}--\eqref{eq:dmp_left2_as} is asymptotically stable and converges to $\hat{\bfx}^p$, we have to prove that $\dot{V}^p(\bfx^p)<0$ for each state $\bfx^p\neq\hat{\bfx}^p$ and that $\dot{V}^p(\bfx^p)=0$ at $\hat{\bfx}^p$. The time derivative of $V^p(\bfx^p)$ can be written as:
\begin{equation*}
\small
\begin{split}
\dot{V}^p(\bfx^p) &= {\cancel{-\bfv_r\tr\bfK(\bfg^p_r-\bfp_r)}} 
    {\cancel{-\bfv_l\tr\bfK(\bfg^p_l-\bfp_l)}} \\
&    {\cancel{-\bfv_r\tr\bfK_f(\bfg^{p}_{rel}-\bfp_{e})}} + {\cancel{\bfv_l\tr\bfK_f(\bfg^{p}_{rel}-\bfp_{e})}} \\
 &  + \bfv_r\tr\left[{\cancel{\bfK(\bfg^p_r - \bfp_r)}} -\bfD\bfv_r +{\cancel{\bfK_f(\bfg^{p}_{rel} - \bfp_{e})}} - \bfD_f\bfv_{e}\right]\\
 &  + \bfv_l\tr\left[{\cancel{\bfK(\bfg^p_l - \bfp_l)}} -\bfD\bfv_l -{\cancel{\bfK_f(\bfg^{p}_{rel} - \bfp_{e})}} + \bfD_f\bfv_{e}\right],
\end{split}
\normalsize
\end{equation*}
where $\bfv_{e} = \bfv_{r} - \bfv_{l}$. After some algebraic operations we obtain:
\begin{equation*}
\small
\begin{split}
\dot{V}^p(\bfx^p) &= -\bfv_r\tr\bfD\bfv_r -\bfv_l\tr\bfD\bfv_l -\bfv_r\tr\bfD_f\bfv_r -\bfv_l\tr\bfD_f\bfv_l + 2\bfv_r\tr\bfD_f\bfv_l \\
 &= -\bfv_r\tr\bfD\bfv_r -\bfv_l\tr\bfD\bfv_l - (\bfv_r-\bfv_l)\tr\bfD_f(\bfv_r-\bfv_l) \leq 0,
\end{split}
\normalsize
\end{equation*}
where $\dot{V}^p(\bfx^p)=0$ if and only if $\bfv_r = \bfv_l = \bfzero$. The LaSalle's invariance theorem \cite{Slotine91} allows to conclude the stability of the system \eqref{eq:dmp_right1_as}--\eqref{eq:dmp_left2_as} and, as a consequence, the stability of the position part of C-DMPs. 

As for the position, the stability of the orientation part of C-DMPs, i.e. the stability of the system \eqref{eq:dmp_ori_right1}--\eqref{eq:dmp_ori_relative2} with coupling forces \eqref{eq:synchro_force_rot1}, \eqref{eq:synchro_force_rot2}, can be proved considering the asymptotic behavior of \eqref{eq:dmp_ori_right1}--\eqref{eq:synchro_force_rot2}. First, we notice that the relative DMP in \eqref{eq:dmp_ori_relative1} and \eqref{eq:dmp_ori_relative2} is decoupled from the other equations, and that the terms $\bff^{q}_{rel}(s)$ and $\bfd^{q,0}_{rel}$ are bounded and vanish for $t\rightarrow+\infty$. Hence, the asymptotic behavior of the relative DMP is given by:
\begin{subequations}
\small
\begin{align}
\dot{\bfq}_{rel} &= \frac{1}{2}\tilde{\bfomega}_{rel} \ast \bfq_{rel}  \label{eq:dmp_ori_rel_as1}\\
\dot{\bfomega}_{rel} &= 2\bfK\log(\bfg^q_{rel} \ast \overline{\bfq}_{rel}) -\bfD\bfomega_{rel}\label{eq:dmp_ori_rel_as2}
\end{align}
\normalsize
\end{subequations}
In order to prove the stability of \eqref{eq:dmp_ori_rel_as1}--\eqref{eq:dmp_ori_rel_as2}, we consider the candidate Lyapunov function:
\begin{equation}
\small
\begin{split}
V^{q}_{rel}(\bfx^q_{rel}) &= V_e(\bfg^q_{rel},\bfq_{rel}) + \frac{1}{2}\bfomega_{rel}\tr\bfomega_{rel}\\
&=\left(\eta_g - \eta_{rel}\right)^2 + \Vert\bfepsilon_g-\bfepsilon_{rel}\Vert^2 + \frac{1}{2}\bfomega_{rel}\tr\bfomega_{rel}\label{eq:lyapunov_fun_rel_ori}
\end{split}
\normalsize
\end{equation}
where the state $\bfx^q_{rel} = [\bfq_{rel}\tr,\,\bfomega_{rel}\tr]\tr$, $\bfq_{rel} = [\eta_{rel},\,\bfepsilon_{rel}\tr]\tr$, and $\bfg^{q}_{rel} = [\eta_g,\,\bfepsilon_{g}\tr]\tr$. The candidate Lyapunov function in \eqref{eq:lyapunov_fun_rel_ori} is positive definite and it vanishes only at the equilibrium $\hat{\bfx}^{q}_{rel} = [{\bfg^{q}_{rel}}\tr,\,\bfzero\tr]\tr$. The time derivative of $V^q_{rel}(\bfx^q_{rel})$ can be written as:
\begin{equation*}
\small
\begin{split}
\dot{V}^{q}_{rel} &= -2\left(\eta_g - \eta_{rel}\right)\dot{\eta}_{rel} -2\left(\bfepsilon_g-\bfepsilon_{rel}\right)\dot{\bfepsilon}_{rel}+\bfomega_{rel}\tr\dot{\bfomega}_{rel}\\
&= \left(\eta_g - \eta_{rel}\right)\bfepsilon_{rel}\tr\bfomega_{rel} + \left(\bfepsilon_g-\bfepsilon_{rel}\right)\tr\left(\eta_{rel}\bfI - \bfS(\bfepsilon_{rel})\right)\bfomega_{rel}\\
&\quad+\bfomega_{rel}\tr\dot{\bfomega}_{rel}
\end{split}
\normalsize
\end{equation*}
where we used the quaternion propagation \eqref{eq:quaternion_propagation}. Considering the definition of $\dot{\bfomega}_{rel}$ in \eqref{eq:dmp_ori_rel_as2}, we obtain that
\begin{equation*}
\small
\begin{split}
\dot{V}^{q}_{rel}&= \left(\eta_g - \eta_{rel}\right)\bfepsilon_{rel}\tr\bfomega_{rel} + \left(\bfepsilon_g-\bfepsilon_{rel}\right)\left(\eta_{rel}\bfI - \bfS(\bfepsilon_{rel})\right)\bfomega_{rel}\\
&\quad+2\bfomega_{rel}\tr\bfK\log(\bfg^q_{rel} \ast \overline{\bfq}_{rel}) -\bfomega_{rel}\tr\bfD\bfomega_{rel}
\end{split}
\normalsize
\end{equation*}
Considering the definition of the quaternion product in \eqref{eq:quaternion_product} and recalling that $\bfS(\bfa)\bfa = \bfzero$, after some algebra we obtain: 
\small
\begin{equation}
\dot{V}^{q}_{rel} = -\bfomega_{rel}\tr\bfD\bfomega_{rel} + \bfomega_{rel}\tr\left(2\bfK\log(\bfg^q_{rel} \ast \overline{\bfq}_{rel}) - \text{vec}(\bfg^q_{rel} \ast \overline{\bfq}_{rel})\right) 
\label{eq:V_dot_ori_rel}
\end{equation}
\normalsize
where the function $\text{vec}(\bfq)$ returns the vector part of the quaternion $\bfq$. Considering the definition of the logarithmic map in \eqref{eq:logarithmic_map}, we can choose
\begin{equation*}
\small
\bfK = \frac{\Vert \text{vec}(\bfg^q_{rel} \ast \overline{\bfq}_{rel})\Vert}{2\arccos(\text{scal}(\bfg^q_{rel} \ast \overline{\bfq}_{rel}))}\bfI \longrightarrow \dot{V}^{q}_{rel} = -\bfomega_{rel}\tr\bfD\bfomega_{rel} \leq 0
\normalsize
\end{equation*} 
where the function $\text{scal}(\bfq)$ returns the scalar part of the quaternion $\bfq$. The derivative of the Lyapunov function is negative semidefinite and it vanishes if and only if $\bfomega_{rel} = \bfzero$. The LaSalle's invariance theorem \cite{Slotine91} allows to conclude the stability of the system \eqref{eq:dmp_ori_rel_as1}--\eqref{eq:dmp_ori_rel_as2}. A useful result derived during the stability analysis is that %
{\small
\begin{equation}
\dot{V}_{e}(\bfg,\bfq) =  -\bfomega_q\tr\text{vec}(\bfg\ast\overline{\bfq})
\label{eq:Ve_dot}
\end{equation}
\normalsize}%
where $\bfg$ is a constant quaternion, $\bfq$ is a time varying quaternion, and $\bfomega_q$ is the angular velocity associated to $\bfq$. This result will be exploited to prove the stability of the orientation part of C-DMPs.

It is worth noticing that previous steps can be used to prove the stability of the Cartesian orientation DMP proposed in  \cite{Ude14}, where a stability proof is missing. Another popular choice for the orientation error is $\text{vec}(\bfg^q_{rel} \ast \overline{\bfq}_{rel})$ \cite{Weitschat16, Pastor11}. The stability of the orientation DMPs proposed in Pastor et al. \cite{Pastor11} can be shown by substituting $2\log(\bfg^q_{rel} \ast \overline{\bfq}_{rel})$ with $\text{vec}(\bfg^q_{rel} \ast \overline{\bfq}_{rel})$ in \eqref{eq:V_dot_ori_rel}, we can guarantee  $\dot{V}^{q}_{rel} \leq 0$ by choosing, for example, $\bfK=\bfI$. This proves that the orientation DMP presented in \cite{Pastor11} is also stable. As experimentally shown in \cite{Ude14}, this choice of the error causes slower convergence to the goal. Hence, we preferred to use the error definition suggested in \cite{Ude14}.  

Having proved the stability of the relative DMP in \eqref{eq:dmp_ori_relative1}--\eqref{eq:dmp_ori_relative2}, we can rewrite the asymptotic behavior of \eqref{eq:dmp_ori_right1}--\eqref{eq:dmp_ori_left2} as:
\begin{subequations}
\small
\begin{align}
\dot{\bfq}_r &= \frac{1}{2}\tilde{\bfomega}_r \ast \bfq_r  \label{eq:dmp_ori_right1_as}\\
\dot{\bfomega}_r &= \bfK\bfe_r -\bfD\bfomega_r  + \bfK_f \bfe_{rel} - \bfD_f\bfomega_e
\label{eq:dmp_ori_right2_as}\\
\dot{\bfq}_l &= \frac{1}{2}\tilde{\bfomega}_l \ast \bfq_l \label{eq:dmp_ori_left1_as}\\
\dot{\bfomega}_l &= \bfK\bfe_l -\bfD\bfomega_l - \bfK_f \bfe_{rel} + \bfD_f\bfomega_e
\label{eq:dmp_ori_left2_as}
\end{align}
\normalsize
\end{subequations}
where we put $\bfomega_e = \bfomega_r - \bfomega_l$, $\bfe_r = 2\log(\bfg^q_r \ast \overline{\bfq}_r)$, $\bfe_l = 2\log(\bfg^q_l \ast \overline{\bfq}_l)$, and $\bfe_{rel} = 2 \log{(\bfg^{q}_{rel} \ast (\overline{\bfq_r\ast\overline{\bfq}_l}) )}$.

In order to prove the stability of \eqref{eq:dmp_ori_right1_as}--\eqref{eq:dmp_ori_left2_as}, we consider the candidate Lyapunov function:
\begin{equation}
\small
\begin{split}
V^{q}(\bfx^q) &= V_e(\bfg^{q}_{r},\bfq_r) + \frac{1}{2}\bfomega_{r}\tr\bfomega_{r} + V_e(\bfg^{q}_{l},\bfq_l) + \frac{1}{2}\bfomega_{l}\tr\bfomega_{l}\\
&\quad+V_e(\bfg^{q}_{rel},\bfq_r\ast\overline{\bfq}_l)
\label{eq:lyapunov_fun_ori}
\end{split}
\normalsize
\end{equation}
where $V_e(\bfq_1,\bfq_2)=\left(\eta_1 - \eta_{2}\right)^2 + \Vert\bfepsilon_1-\bfepsilon_2\Vert^2$ is defined as in \eqref{eq:lyapunov_fun_rel_ori} and the state $\bfx^q = [\bfq_{r}\tr,\,\bfq_{l}\tr,\,\bfomega_{r}\tr,\,\bfomega_{l}\tr]\tr$. The candidate Lyapunov function in \eqref{eq:lyapunov_fun_rel_ori} is positive definite and it vanishes only at the equilibrium $\hat{\bfx}^{q} = [{\bfg^{q}_{r}}\tr,\,{\bfg^{q}_{l}}\tr,\,\bfzero\tr,\,\bfzero\tr]\tr$ if and only if $\bfg^{q}_{rel} = \bfg^{q}_{r}\ast\overline{\bfg}^{q}_l$. The time derivative of $V^q(\bfx^q)$ can be written as:
\begin{equation}
\small
\begin{split}
\dot{V}^{q}(\bfx^q) &= \dot{V}_e(\bfg^{q}_{r},\bfq_r) + \bfomega_{r}\tr[\bfK\bfe_r -\bfD\bfomega_r  + \bfK_f \bfe_{rel} - \bfD_f\bfomega_e]\\
              &\quad\dot{V}_e(\bfg^{q}_{l},\bfq_l)+ \bfomega_{l}\tr[\bfK\bfe_l -\bfD\bfomega_l - \bfK_f \bfe_{rel} + \bfD_f\bfomega_e]\\
              &\quad+\dot{V}_e(\bfg^{q}_{rel},\bfq_r\ast\overline{\bfq}_l)
\label{eq:dot_lyapunov_fun_ori}
\end{split}
\normalsize
\end{equation}
where we used the definitions of $\dot{\bfomega}_{r}$ and $\dot{\bfomega}_{l}$ in \eqref{eq:dmp_ori_right2_as} and \eqref{eq:dmp_ori_left2_as} respectively. %Following similar steps as in \eqref{eq:V_dot_ori_rel} and 
Considering the expression of $\dot{V}_e$ in \eqref{eq:Ve_dot}, and recalling that $\bfomega_e=\bfomega_r-\bfomega_l$ is the angular velocity associated to the quaternion $\bfq_r\ast\overline{\bfq}_l$, it is possible to rewrite \eqref{eq:dot_lyapunov_fun_ori} as:
\begin{equation}
\small
\begin{split}
\dot{V}^{q}(\bfx^q) &= -\bfomega_{r}\tr\bfD\bfomega_{r} + \bfomega_{r}\tr\left(\bfK_r\bfe_r - \text{vec}(\bfg^q_{r} \ast \overline{\bfq}_{r})\right) \\
              &\quad-\bfomega_{l}\tr\bfD\bfomega_{l} + \bfomega_{l}\tr\left(\bfK_l\bfe_l - \text{vec}(\bfg^q_{l} \ast \overline{\bfq}_{l})\right) \\
              &\quad-\bfomega_{e}\tr\bfD_f\bfomega_{e} + \bfomega_{e}\tr\left(\bfK_f \bfe_{rel} - \text{vec}(\bfg^{q}_{rel}\ast\left(\overline{\bfq_r\ast\overline{\bfq}_l}\right)\right)
\label{eq:dot_lyapunov_fun_ori2}
\end{split}
\normalsize
\end{equation}
By choosing 
\begin{equation*}
\small
\begin{split}
&\bfK_r = \frac{\Vert \text{vec}(\bfg^q_{r} \ast \overline{\bfq}_{r})\Vert}{2\arccos(\text{scal}(\bfg^q_{r} \ast \overline{\bfq}_{r}))}\bfI, \quad \bfK_l = \frac{\Vert \text{vec}(\bfg^q_{l} \ast \overline{\bfq}_{l})\Vert}{2\arccos(\text{scal}(\bfg^q_{l} \ast \overline{\bfq}_{l}))}\bfI,\\
&\text{and}\quad\bfK_f = \frac{\Vert\text{vec}\left(\bfg^{q}_{rel}\ast\left(\overline{\bfq_r\ast\overline{\bfq}_l}\right)\right)\Vert}{2\arccos\left(\text{scal}\left(\bfg^{q}_{rel}\ast\left(\overline{\bfq_r\ast\overline{\bfq}_l}\right)\right)\right)}\bfI,
\end{split}
\normalsize
\end{equation*} 
the derivative of the Lyapunov function becomes
\begin{equation*}
\small
\begin{split}
\dot{V}^{q}(\bfx^q) = -\bfomega_{r}\tr\bfD\bfomega_{r} -\bfomega_{l}\tr\bfD\bfomega_{l} -\bfomega_{e}\tr\bfD_f\bfomega_{e} \leq 0
\end{split}
\normalsize
\end{equation*}
The derivative of the Lyapunov function is negative semidefinite and it vanishes if and only if $\bfomega_{r} = \bfomega_{l} = \bfzero$. The LaSalle's invariance theorem \cite{Slotine91} allows to conclude the stability of the system \eqref{eq:dmp_ori_right1_as}--\eqref{eq:dmp_ori_left2_as} and, as a consequence, the stability of the orientation part of C-DMPs.

The conducted stability analysis \textcolor{red}{tells N things ... Say about relative goal, K and D diagonal}

Given the orientation stiffness gains $\bfK = k\bfI$, the orientation damping gains $\bfD = d\bfI$ are chosen as $\bfD = \sqrt{4k}\bfI$ to have a critically damped system \cite{Weitschat16}.

The original DMPs contain a constant scaling term ($\tau > 0$) used to speed-up or slow-down the motion execution \cite{DMP}. The scaling term can be eventually added to the C-DMPs without compromising the stability

%and considering the relation
%\begin{equation*}
%\small
%\dot{V}_e(\bfg^{q}_{rel},\bfq_r\ast\overline{\bfq}_l) = -\bfomega_e\tr\text{vec}\left(\overline{\bfq_r\ast\overline{\bfq}_l}\right),
%\normalsize
%\end{equation*} 
%
%\begin{equation}
%\small
%\begin{split}
%\dot{V}^{q}(\bfx^q) &= -2\left(\eta^g_r - \eta_{r}\right)\dot{\eta}_{r} -2 (\bfepsilon^g_r-\bfepsilon_{r})\tr\dot{\bfepsilon}_{r} + \bfomega_{r}\tr\dot{\bfomega}_{r}\\
%              &\quad-2\left(\eta^g_l - \eta_{l}\right)\dot{\eta}_{l} -2 (\bfepsilon^g_l-\bfepsilon_{l})\tr\dot{\bfepsilon}_{l} + \bfomega_{l}\tr\dot{\bfomega}_{l}\\
%              &= -\left(\eta^g_r - \eta_{r}\right)\bfepsilon_{r}\tr\bfomega_r - (\bfepsilon^g_r-\bfepsilon_{r})\tr\left(\eta_{r}\bfI - \bfS(\bfepsilon_{r})\right)\bfomega_{r} + \bfomega_{r}\tr\dot{\bfomega}_{r}\\
%              &\quad-\left(\eta^g_l - \eta_{l}\right)\bfepsilon_{l}\tr\bfomega_l - (\bfepsilon^g_l-\bfepsilon_{l})\tr\left(\eta_{l}\bfI - \bfS(\bfepsilon_{l})\right)\bfomega_{l} + \bfomega_{l}\tr\dot{\bfomega}_{l}
%\label{eq:dot_lyapunov_fun_ori}
%\end{split}
%\normalsize
%\end{equation}

==> sections/Related_Work.tex <==
\section{Related Work}
Symmetric and asymmetric bimanual control []

\cite{Denisa16, Batinica17}

==> sections/Stability_proof/Case1.tex <==
\subsection*{Case I} In this case, coupling forces are defined as:
\begin{subequations}
\small
\begin{align}
\bff^p_{r,l} &= \bff^p_{l,r} = \bff^q_{r,l} = \bff^q_{l, r} = \bfzero, \label{eq:synchro_force_1_1}\\
\bff^v_{r,l} &= \bfK_f(\bfp_{rel} - \bfp_{r,l}) + \bfD_f(\bfv_{rel} - \bfv_{r,l}), \label{eq:synchro_force_1_2}\\
\bff^v_{l,r} &= -\bff^v_{r,l},\label{eq:synchro_force_1_3}\\
\bff^{\omega}_{r,l} &= \bfK_f 2 \text{vec}{(\bfq_{rel} \ast \overline{\bfq}_{r,l} )} + \bfD_f(\bfomega_{rel} - \bfomega_{r,l}),\label{eq:synchro_force_1_4}\\
\bff^{\omega}_{l,r} &= \bfK_f 2 \text{vec}{(\overline{\bfq}_{rel} \ast \overline{\bfq}_{l,r})} - \bfD_f(\bfomega_{rel} - \bfomega_{r,l}).\label{eq:synchro_force_1_5}
\end{align}
\normalsize
\end{subequations}
where in \eqref{eq:synchro_force_1_5} we used $\bfomega_{r,l} = -\bfomega_{l,r}$ and considered that $\bfq_{rel}$ and $\bfomega_{rel}$ are expressed in the right hand frame.

Let us first focus on the position, i.e. on the stability of the system of differential equations \eqref{eq:dmp_right1}--\eqref{eq:dmp_relative2} with coupling forces defined as in \eqref{eq:synchro_force_1_1}--\eqref{eq:synchro_force_1_3}. First, we notice that the relative DMP in \eqref{eq:dmp_relative1}, \eqref{eq:dmp_relative2} is  decoupled from the other differential equations, and that the terms $\bff^{p}_{rel}(s)$ and $\bfd^{p,0}_{rel}$ are bounded and vanish for $t\rightarrow+\infty$. This implies that the relative DMP is stable ($\bfp_{rel}\rightarrow\bfg^{p}_{rel}$ and $\bfv_{rel}\rightarrow\bfzero$) if the gain matrices $\bfK$ and $\bfD$ are positive definite. Given this, and considering that the nonlinear terms $\bff^{p}_{r}(s)$ and $\bff^{p}_{l}(s)$ are bounded and vanish for $t\rightarrow+\infty$, we can conclude the stability of C-DMPs by analyzing the asymptotic behavior of \eqref{eq:dmp_right1}--\eqref{eq:dmp_left2}. For $t\rightarrow+\infty$, we can rewrite \eqref{eq:synchro_force_1_2} and \eqref{eq:synchro_force_1_3} as:
\begin{subequations}
\small
\begin{align}
\bff^p_{r,l} &= \bfK_f(\bfg^{p}_{rel} - \bfp_{r,l}) - \bfD_f\bfv_{r,l}\label{eq:synchro_force1_as}\\
\bff^p_{l,r} &= -\bff^p_{r,l} = -\bfK_f(\bfg^{p}_{rel} - \bfp_{r,l}) + \bfD_f\bfv_{r,l} \label{eq:synchro_force2_as}
\end{align}
\normalsize
\end{subequations}
and \eqref{eq:dmp_right1}--\eqref{eq:dmp_left2} as:
\begin{subequations}
\small
\begin{align}
\dot{\bfp}_r &= \bfv_r \label{eq:dmp_right1_as}\\
\dot{\bfv}_r &= \bfK(\bfg^p_r - \bfp_r)-\bfD\bfv_r +\bfK_f(\bfg^{p}_{rel} - \bfp_{r,l}) - \bfD_f\bfv_{r,l}\label{eq:dmp_right2_as}\\
\dot{\bfp}_l &= \bfv_l \label{eq:dmp_left1_as}\\
\dot{\bfv}_l &= \bfK(\bfg^p_l - \bfp_l) -\bfD\bfv_l -\bfK_f(\bfg^{p}_{rel} - \bfp_{r,l}) + \bfD_f\bfv_{r,l}\label{eq:dmp_left2_as}
\end{align}
\end{subequations}
\normalsize
In order to prove the stability of \eqref{eq:dmp_right1_as}--\eqref{eq:dmp_left2_as}, we consider the candidate Lyapunov function:
\begin{equation}
\small
\begin{split}
V^p(\bfx^p) &= \frac{1}{2}(\bfg^p_r-\bfp_r)\tr\bfK(\bfg^p_r-\bfp_r) +
    \frac{1}{2}(\bfg^p_l-\bfp_l)\tr\bfK(\bfg^p_l-\bfp_l) \\
    &\quad+\frac{1}{2}(\bfg^{p}_{rel}-\bfp_{r,l})\tr\bfK_f(\bfg^{p}_{rel}-\bfp_{r,l}) +
    \frac{1}{2}\bfv_r\tr\bfv_r + \frac{1}{2}\bfv_l\tr\bfv_l\label{eq:lyapunov_fun}
\end{split}
\normalsize
\end{equation}
where the state is defined as $\bfx^p = [\bfp_r\tr,\, \bfp_l\tr,\, \bfv_r\tr,\, \bfv_l\tr]\tr\in\mathbb{R}^{12}$.  The candidate Lyapunov function in \eqref{eq:lyapunov_fun} is positive definite if $\bfK$ and $\bfK_f$ are positive definite matrices, and it vanishes only at the equilibrium point $\hat{\bfx}^p =[{\bfg^{p}_{r}}\tr,\, {\bfg^{p}_{l}}\tr,\, \bfzero\tr,\, \bfzero\tr]\tr$ if and only if $\bfg^{p}_{r}-\bfg^{p}_{l} = \bfg^{p}_{rel}$. To show that $V^p(\bfx^p)$ is a proper Lyapunov function, which implies that the system \eqref{eq:dmp_right1_as}--\eqref{eq:dmp_left2_as} is asymptotically stable and converges to $\hat{\bfx}^p$, we have to prove that $\dot{V}^p(\bfx^p)<0$ for each state $\bfx^p\neq\hat{\bfx}^p$ and that $\dot{V}^p(\bfx^p)=0$ at $\hat{\bfx}^p$. The time derivative of $V^p(\bfx^p)$ can be written as:
\begin{equation*}
\small
\begin{split}
\dot{V}^p(\bfx^p) &= {\cancel{-\bfv_r\tr\bfK(\bfg^p_r-\bfp_r)}} 
    {\cancel{-\bfv_l\tr\bfK(\bfg^p_l-\bfp_l)}} \\
&    {\cancel{-\bfv_r\tr\bfK_f(\bfg^{p}_{rel}-\bfp_{r,l})}} + {\cancel{\bfv_l\tr\bfK_f(\bfg^{p}_{rel}-\bfp_{r,l})}} \\
 &  + \bfv_r\tr\left[{\cancel{\bfK(\bfg^p_r - \bfp_r)}} -\bfD\bfv_r +{\cancel{\bfK_f(\bfg^{p}_{rel} - \bfp_{r,l})}} - \bfD_f\bfv_{r,l}\right]\\
 &  + \bfv_l\tr\left[{\cancel{\bfK(\bfg^p_l - \bfp_l)}} -\bfD\bfv_l -{\cancel{\bfK_f(\bfg^{p}_{rel} - \bfp_{r,l})}} + \bfD_f\bfv_{r,l}\right],
\end{split}
\normalsize
\end{equation*}
After some algebraic operations, and recalling that $\bfv_{r,l} = \bfv_{r} - \bfv_{l}$, we obtain:
\begin{equation*}
\small
\begin{split}
\dot{V}^p(\bfx^p) &= -\bfv_r\tr\bfD\bfv_r -\bfv_l\tr\bfD\bfv_l -\bfv_r\tr\bfD_f\bfv_r -\bfv_l\tr\bfD_f\bfv_l + 2\bfv_r\tr\bfD_f\bfv_l \\
 &= -\bfv_r\tr\bfD\bfv_r -\bfv_l\tr\bfD\bfv_l - (\bfv_r-\bfv_l)\tr\bfD_f(\bfv_r-\bfv_l) \leq 0,
\end{split}
\normalsize
\end{equation*}
where $\dot{V}^p(\bfx^p)=0$ if and only if $\bfv_r = \bfv_l = \bfzero$. The LaSalle's invariance theorem \cite{Slotine91} allows to conclude the stability of the system \eqref{eq:dmp_right1_as}--\eqref{eq:dmp_left2_as} and, as a consequence, the stability of the position part of C-DMPs. 

Despite the nonlinearity introduced by the quaternion propagation and quaternion error, the stability of the orientation part of C-DMPs, i.e. the stability of the system \eqref{eq:dmp_ori_right1}--\eqref{eq:dmp_ori_relative2} with coupling forces \eqref{eq:synchro_force_1_1}, \eqref{eq:synchro_force_1_4}, and \eqref{eq:synchro_force_1_4}, can be proved considering the asymptotic behavior of \eqref{eq:dmp_ori_right1}--\eqref{eq:dmp_ori_relative2}. The reason is that the orientation part of C-DMPs can be considered as an \textit{asymptotically autonomous differential system} \cite{Markus56}.


First, we notice that the relative DMP in \eqref{eq:dmp_ori_relative1} and \eqref{eq:dmp_ori_relative2} is decoupled from the other equations, and that the terms $\bff^{q}_{rel}(s)$ and $\bfd^{q,0}_{rel}$ are bounded and vanish for $t\rightarrow+\infty$. Hence, the asymptotic behavior of the relative DMP is given by:
\begin{subequations}
\small
\begin{align}
\dot{\bfq}_{rel} &= \frac{1}{2}\tilde{\bfomega}_{rel} \ast \bfq_{rel}  \label{eq:dmp_ori_rel_as1}\\
\dot{\bfomega}_{rel} &= 2\bfK\text{vec}(\bfg^q_{rel} \ast \overline{\bfq}_{rel}) -\bfD\bfomega_{rel}\label{eq:dmp_ori_rel_as2}
\end{align}
\normalsize
\end{subequations}
In order to prove the stability of \eqref{eq:dmp_ori_rel_as1}--\eqref{eq:dmp_ori_rel_as2}, we consider the candidate Lyapunov function:
\begin{equation}
\small
\begin{split}
V^{q}_{rel}(\bfx^q_{rel}) &= V_e(\bfg^q_{rel},\bfq_{rel}) + \frac{1}{4}\bfomega_{rel}\tr\bfK^{-1}\bfomega_{rel}\\
&=\left(\eta_g - \eta_{rel}\right)^2 + \Vert\bfepsilon_g-\bfepsilon_{rel}\Vert^2 + \frac{1}{4}\bfomega_{rel}\tr\bfK^{-1}\bfomega_{rel}\label{eq:lyapunov_fun_rel_ori}
\end{split}
\normalsize
\end{equation}
where the state $\bfx^q_{rel} = [\bfq_{rel}\tr,\,\bfomega_{rel}\tr]\tr$, $\bfq_{rel} = [\eta_{rel},\,\bfepsilon_{rel}\tr]\tr$, and $\bfg^{q}_{rel} = [\eta_g,\,\bfepsilon_{g}\tr]\tr$. The candidate Lyapunov function in \eqref{eq:lyapunov_fun_rel_ori} is positive definite and it vanishes only at the equilibrium $\hat{\bfx}^{q}_{rel} = [{\bfg^{q}_{rel}}\tr,\,\bfzero\tr]\tr$. The time derivative of $V^q_{rel}(\bfx^q_{rel})$ can be written as:
\begin{equation*}
\small
\begin{split}
\dot{V}^{q}_{rel} &= -2\left(\eta_g - \eta_{rel}\right)\dot{\eta}_{rel} -2\left(\bfepsilon_g-\bfepsilon_{rel}\right)\dot{\bfepsilon}_{rel}+\bfomega_{rel}\tr\bfK^{-1}\dot{\bfomega}_{rel}\\
&= \left(\eta_g - \eta_{rel}\right)\bfepsilon_{rel}\tr\bfomega_{rel} + \left(\bfepsilon_g-\bfepsilon_{rel}\right)\tr\left(\eta_{rel}\bfI - \bfS(\bfepsilon_{rel})\right)\bfomega_{rel}\\
&\quad+\frac{1}{2}\bfomega_{rel}\tr\bfK^{-1}\dot{\bfomega}_{rel}
\end{split}
\normalsize
\end{equation*}
where we used \eqref{eq:dmp_ori_rel_as1} and the quaternion propagation \eqref{eq:quaternion_propagation}. Considering the definition of $\dot{\bfomega}_{rel}$ in \eqref{eq:dmp_ori_rel_as2}, we obtain that
\begin{equation*}
\small
\begin{split}
\dot{V}^{q}_{rel}&= \left(\eta_g - \eta_{rel}\right)\bfepsilon_{rel}\tr\bfomega_{rel} + \left(\bfepsilon_g-\bfepsilon_{rel}\right)\left(\eta_{rel}\bfI - \bfS(\bfepsilon_{rel})\right)\bfomega_{rel}\\
&\quad+\bfomega_{rel}\tr\cancel{\bfK^{-1}\bfK}\text{vec}(\bfg^q_{rel} \ast \overline{\bfq}_{rel}) -\frac{1}{2}\bfomega_{rel}\tr\bfK^{-1}\bfD\bfomega_{rel}
\end{split}
\normalsize
\end{equation*}
Note that the matrix $\bfK^{-1}\bfD$, obtained by multiplying the two positive definite matrices $\bfK^{-1}$ and $\bfD$, is positive definite iff $\bfK^{-1}\bfD = \bfD\bfK^{-1}$. This property can be guaranteed, for example, by assuming that $\bfK$ and $\bfD$ are diagonal matrices. In the rest of the analysis, we assume that  $\bfD_k = \bfK^{-1}\bfD$ is a positive definite matrix.  Considering the definition of the quaternion product in \eqref{eq:quaternion_product} and recalling that $\bfS(\bfa)\bfa = \bfzero$, after some algebra we obtain: 
\begin{equation*}
\small
\begin{split}
\dot{V}^{q}_{rel} &= -\frac{1}{2}\bfomega_{rel}\tr\bfD_k\bfomega_{rel} + \bfomega_{rel}\tr\left(\text{vec}(\bfg^q_{rel} \ast \overline{\bfq}_{rel}) - \text{vec}(\bfg^q_{rel} \ast \overline{\bfq}_{rel})\right) \\
 &= -\frac{1}{2}\bfomega_{rel}\tr\bfD_k\bfomega_{rel} \leq 0
%\label{eq:V_dot_ori_rel}
\end{split}
\normalsize
\end{equation*}
%where the function $\text{vec}(\bfq)$ returns the vector part of the quaternion $\bfq$. Considering the definition of the logarithmic map in \eqref{eq:logarithmic_map}, we can choose
%\begin{equation*}
%\small
%\bfK = \frac{\Vert \text{vec}(\bfg^q_{rel} \ast \overline{\bfq}_{rel})\Vert}{2\arccos(\text{scal}(\bfg^q_{rel} \ast \overline{\bfq}_{rel}))}\bfI \longrightarrow \dot{V}^{q}_{rel} = -\bfomega_{rel}\tr\bfD\bfomega_{rel} \leq 0
%\normalsize
%\end{equation*} 
%where the function $\text{scal}(\bfq)$ returns the scalar part of the quaternion $\bfq$. 
The derivative of the Lyapunov function is negative semidefinite and it vanishes if and only if $\bfomega_{rel} = \bfzero$. The LaSalle's invariance theorem \cite{Slotine91} allows to conclude the stability of the system \eqref{eq:dmp_ori_rel_as1}--\eqref{eq:dmp_ori_rel_as2}. A useful result derived during the stability analysis is that %
{\small
\begin{equation}
\dot{V}_{e}(\bfg,\bfq) =  -\bfomega\tr\text{vec}(\bfg\ast\overline{\bfq}) = -\frac{1}{2}\bfomega\tr\bfe
\label{eq:Ve_dot}
\end{equation}
\normalsize}%
where $\bfg$ is a constant quaternion, $\bfq$ is a time varying quaternion, $\bfomega$ is the angular velocity associated to $\bfq$, and $\bfe$ is the orientation error between $\bfg$ and $\bfq$. This result will be exploited to prove the stability of the orientation part of C-DMPs.

%It is worth noticing that previous steps can be used to prove the stability of the Cartesian orientation DMP proposed in  \cite{Ude14}, where a stability proof is missing. Another popular choice for the orientation error is $\text{vec}(\bfg^q_{rel} \ast \overline{\bfq}_{rel})$ \cite{Weitschat16, Pastor11}. The stability of the orientation DMPs proposed in Pastor et al. \cite{Pastor11} can be shown by substituting $2\text{vec}(\bfg^q_{rel} \ast \overline{\bfq}_{rel})$ with $\text{vec}(\bfg^q_{rel} \ast \overline{\bfq}_{rel})$ in \eqref{eq:V_dot_ori_rel}, we can guarantee  $\dot{V}^{q}_{rel} \leq 0$ by choosing, for example, $\bfK=\bfI$. This proves that the orientation DMP presented in \cite{Pastor11} is also stable. As experimentally shown in \cite{Ude14}, this choice of the error causes slower convergence to the goal. Hence, we preferred to use the error definition suggested in \cite{Ude14}.  
It is worth noticing that previous steps can be used to prove the stability of the Cartesian orientation DMP proposed in \cite{Pastor11}, where a stability proof is missing. Another possible choice for the orientation error is $\bfe = 2\text{log}(\bfg \ast \overline{\bfq})$ \cite{Ude14}, where the logarithmic map is defined as in \eqref{eq:logarithmic_map}. The stability of the orientation DMPs proposed by Ude et al. \cite{Ude14} can be shown using $V^{q} = V_e(\bfg,\bfq) + 0.5\bfomega\tr\bfomega$ as Lyapunov candidate and selecting $\bfK = \frac{\Vert \text{vec}(\bfg \ast \overline{\bfq})\Vert}{2\arccos(\text{scal}(\bfg \ast \overline{\bfq}))}\bfI$ as stiffness gain. In this work, we used the vector-based quaternion error in order to avoid  constraints on the control gain matrices.


% This proves that the orientation DMP presented in \cite{Pastor11} is also stable. As experimentally shown in \cite{Ude14}, this choice of the error causes slower convergence to the goal. Hence, we preferred to use the error definition suggested in \cite{Ude14}.  

Having proved the stability of the relative DMP in \eqref{eq:dmp_ori_relative1}--\eqref{eq:dmp_ori_relative2}, we can rewrite the asymptotic behavior of \eqref{eq:dmp_ori_right1}--\eqref{eq:dmp_ori_left2} as:
\begin{subequations}
\small
\begin{align}
\dot{\bfq}_r &= \frac{1}{2}\tilde{\bfomega}_r \ast \bfq_r  \label{eq:dmp_ori_right1_as}\\
\dot{\bfomega}_r &= \bfK\bfe_r -\bfD\bfomega_r  + \bfK_f \bfe_{r,l} - \bfD_f\bfomega_{r,l}
\label{eq:dmp_ori_right2_as}\\
\dot{\bfq}_l &= \frac{1}{2}\tilde{\bfomega}_l \ast \bfq_l \label{eq:dmp_ori_left1_as}\\
\dot{\bfomega}_l &= \bfK\bfe_l -\bfD\bfomega_l + \bfK_f \bfe_{l,r} + \bfD_f\bfomega_{r,l}
\label{eq:dmp_ori_left2_as}
\end{align}
\normalsize
\end{subequations}
where $\bfe_r = 2\text{vec}(\bfg^q_r \ast \overline{\bfq}_r)$, $\bfe_l = 2\text{vec}(\bfg^q_l \ast \overline{\bfq}_l)$, $\bfe_{r,l} = 2 \text{vec}{(\bfg^{q}_{rel} \ast (\overline{\bfq_r\ast\overline{\bfq}_l}) )}$, and $\bfe_{l,r} = 2 \text{vec}{(\overline{\bfg}^{q}_{rel} \ast (\overline{\bfq_l\ast\overline{\bfq}_r}) )}$.

In order to prove the stability of \eqref{eq:dmp_ori_right1_as}--\eqref{eq:dmp_ori_left2_as}, we consider the candidate Lyapunov function:
\begin{equation}
\small
\begin{split}
V^{q}(\bfx^q) &= 2V_e(\bfg^{q}_{r},\bfq_r) + \frac{1}{2}\bfomega_{r}\tr\bfK^{-1}\bfomega_{r} + 2V_e(\bfg^{q}_{l},\bfq_l) \\
&+ \frac{1}{2}\bfomega_{l}\tr\bfK^{-1}\bfomega_{l}+2V_e(\bfg^{q}_{rel},\bfq_r\ast\overline{\bfq}_l)+2V_e(\overline{\bfg}^{q}_{rel},\bfq_l\ast\overline{\bfq}_r)
\label{eq:lyapunov_fun_ori}
\end{split}
\normalsize
\end{equation}
where $V_e(\bfq_1,\bfq_2)=\left(\eta_1 - \eta_{2}\right)^2 + \Vert\bfepsilon_1-\bfepsilon_2\Vert^2$ and the state $\bfx^q = [\bfq_{r}\tr,\,\bfq_{l}\tr,\,\bfomega_{r}\tr,\,\bfomega_{l}\tr]\tr$. The candidate Lyapunov function in \eqref{eq:lyapunov_fun_rel_ori} is positive definite and it vanishes only at the equilibrium $\hat{\bfx}^{q} = [{\bfg^{q}_{r}}\tr,\,{\bfg^{q}_{l}}\tr,\,\bfzero\tr,\,\bfzero\tr]\tr$ if and only if $\bfg^{q}_{rel} = \bfg^{q}_{r}\ast\overline{\bfg}^{q}_l$. The time derivative of $V^q(\bfx^q)$ can be written as:
\begin{equation}
\small
\begin{split}
\dot{V}^{q}(\bfx^q) &= 2\dot{V}_e(\bfg^{q}_{r},\bfq_r) + 2\dot{V}_e(\bfg^{q}_{l},\bfq_l)\\
&\quad+\bfomega_{r}\tr\bfK^{-1}[\bfK\bfe_r -\bfD\bfomega_r  + \bfK_f \bfe_{r,l} - \bfD_f\bfomega_{r,l}]\\
              &\quad+\bfomega_{l}\tr\bfK^{-1}[\bfK\bfe_l -\bfD\bfomega_l + \bfK_f \bfe_{l,r} + \bfD_f\bfomega_{r,l}]\\
              &\quad+2\dot{V}_e(\bfg^{q}_{rel},\bfq_r\ast\overline{\bfq}_l)+2\dot{V}_e(\overline{\bfg}^{q}_{rel},\bfq_l\ast\overline{\bfq}_r)
\label{eq:dot_lyapunov_fun_ori}
\end{split}
\normalsize
\end{equation}
where we used the definitions of $\dot{\bfomega}_{r}$ and $\dot{\bfomega}_{l}$ in \eqref{eq:dmp_ori_right2_as} and \eqref{eq:dmp_ori_left2_as} respectively. %Following similar steps as in \eqref{eq:V_dot_ori_rel} and 
Considering the general expression  of $\dot{V}_e$ in \eqref{eq:Ve_dot}, and recalling that $\bfomega_{r,l}=\bfomega_r-\bfq_{r,l}\ast\bfomega_l\ast\overline{\bfq}_{r,l}$ is the angular velocity associated to the quaternion $\bfq_{r,l}=\bfq_r\ast\overline{\bfq}_l$, it is possible to rewrite \eqref{eq:dot_lyapunov_fun_ori} as:
\begin{equation}
\small
\begin{split}
\dot{V}^{q}(\bfx^q) &= -\bfomega_{r}\tr\bfD_k\bfomega_{r} -\bfomega_{l}\tr\bfD_k\bfomega_{l} -\bfomega_{r,l}\tr\bfK^{-1}\bfD_f\bfomega_{r,l}\\
&\quad + \bfomega_{r,l}\tr\left(\bfK^{-1}\bfK_f \bfe_{rel} - \text{vec}(\bfg^{q}_{rel}\ast\left(\overline{\bfq_r\ast\overline{\bfq}_l}\right)\right)\\
&\quad + \bfomega_{r,l}\tr\left(\bfK^{-1}\bfK_f \bfe_{rel} - \text{vec}(\bfg^{q}_{rel}\ast\left(\overline{\bfq_r\ast\overline{\bfq}_l}\right)\right)
\label{eq:dot_lyapunov_fun_ori1_2}
\end{split}
\normalsize
\end{equation}
%\begin{equation}
%\small
%\begin{split}
%\dot{V}^{q}(\bfx^q) &= -\frac{1}{2}\bfomega_{r}\tr\bfD_k\bfomega_{r} + \bfomega_{r}\tr\left(\bfe_r - \text{vec}(\bfg^q_{r} \ast \overline{\bfq}_{r})\right) \\
%              &\quad-\bfomega_{l}\tr\bfD\bfomega_{l} + \bfomega_{l}\tr\left(\bfK_l\bfe_l - \text{vec}(\bfg^q_{l} \ast \overline{\bfq}_{l})\right) \\
%              &\quad-\bfomega_{e}\tr\bfD_f\bfomega_{e} + \bfomega_{e}\tr\left(\bfK_f \bfe_{rel} - \text{vec}(\bfg^{q}_{rel}\ast\left(\overline{\bfq_r\ast\overline{\bfq}_l}\right)\right)
%\label{eq:dot_lyapunov_fun_ori2}
%\end{split}
%\normalsize
%\end{equation}
By choosing  $\bfK_f = \bfK$ 
%\begin{equation*}
%\small
%\begin{split}
%&\bfK_r = \frac{\Vert \text{vec}(\bfg^q_{r} \ast \overline{\bfq}_{r})\Vert}{2\arccos(\text{scal}(\bfg^q_{r} \ast \overline{\bfq}_{r}))}\bfI, \quad \bfK_l = \frac{\Vert \text{vec}(\bfg^q_{l} \ast \overline{\bfq}_{l})\Vert}{2\arccos(\text{scal}(\bfg^q_{l} \ast \overline{\bfq}_{l}))}\bfI,\\
%&\text{and}\quad\bfK_f = \frac{\Vert\text{vec}\left(\bfg^{q}_{rel}\ast\left(\overline{\bfq_r\ast\overline{\bfq}_l}\right)\right)\Vert}{2\arccos\left(\text{scal}\left(\bfg^{q}_{rel}\ast\left(\overline{\bfq_r\ast\overline{\bfq}_l}\right)\right)\right)}\bfI,
%\end{split}
%\normalsize
%\end{equation*} 
the derivative of the Lyapunov function becomes
\begin{equation*}
\small
\begin{split}
\dot{V}^{q}(\bfx^q) = -\bfomega_{r}\tr\bfD\bfomega_{r} -\bfomega_{l}\tr\bfD\bfomega_{l} -\bfomega_{r,l}\tr\bfD_f\bfomega_{r,l} \leq 0
\end{split}
\normalsize
\end{equation*}
The derivative of the Lyapunov function is negative semidefinite and it vanishes if and only if $\bfomega_{r} = \bfomega_{l} = \bfzero$. The LaSalle's invariance theorem \cite{Slotine91} allows to conclude the stability of the system \eqref{eq:dmp_ori_right1_as}--\eqref{eq:dmp_ori_left2_as} and, as a consequence, the stability of the orientation part of C-DMPs.

The conducted stability analysis \textcolor{red}{tells N things ... Say about relative goal, K and D diagonal, $K_f = K$}

Given the orientation stiffness gains $\bfK = k\bfI$, the orientation damping gains $\bfD = d\bfI$ are chosen as $\bfD = \sqrt{4k}\bfI$ to have a critically damped system \cite{Weitschat16}.

The original DMPs contain a constant scaling term ($\tau > 0$) used to speed-up or slow-down the motion execution \cite{DMP}. The scaling term can be eventually added to the C-DMPs without compromising the stability


==> sections/Stability_proof/Case2.tex <==
\subsection*{Case II} In this case, coupling forces are defined as:
\begin{subequations}
\small
\begin{align}
\bff^p_{r,l} &= \bfK_f(\bfp_{rel} - \bfp_{r,l}), ~ \bff^p_{l,r} = -\bff^p_{r,l},\label{eq:synchro_force_2_1}\\
\bff^{q}_{r,l} &= \bfK_f 2 \text{vec}{(\bfq_{rel} \ast \overline{\bfq}_{r,l} )}, ~\bff^{q}_{l,r} = -\bfq_{l,r}\ast\bff^{q}_{r,l}\ast\overline{\bfq}_{l,r}, \label{eq:synchro_force_2_2}\\
\quad\bff^v_{r,l} &= \bff^v_{l,r} = \bff^{\omega}_{r,l} = \bff^{\omega}_{l, r} = \bfzero. \label{eq:synchro_force_2_3}
\end{align}
\normalsize
\end{subequations}

Let us first focus on the position, i.e. on the stability of the system of differential equations \eqref{eq:dmp_right1}--\eqref{eq:dmp_relative2} with coupling forces defined as in \eqref{eq:synchro_force_2_1} and \eqref{eq:synchro_force_2_3}. As discussed in Case I, the relative DMP is stable ($\bfp_{rel}\rightarrow\bfg^{p}_{rel}$ and $\bfv_{rel}\rightarrow\bfzero$) if the gain matrices $\bfK$ and $\bfD$ are positive definite, and we can conclude the stability of C-DMPs by analyzing the asymptotic behavior of \eqref{eq:dmp_right1}--\eqref{eq:dmp_left2}. For $t\rightarrow+\infty$, we can rewrite \eqref{eq:dmp_right1}--\eqref{eq:dmp_left2} as:
\begin{subequations}
\small
\begin{align}
\dot{\bfp}_r &= \bfv_r + \bfK_f(\bfg_{rel} - \bfp_{r,l}) \label{eq:dmp_right2_1_as}\\
\dot{\bfv}_r &= \bfK(\bfg^p_r - \bfp_r)-\bfD\bfv_r \label{eq:dmp_right2_2_as}\\
\dot{\bfp}_l &= \bfv_l - \bfK_f(\bfg_{rel} - \bfp_{r,l}) \label{eq:dmp_left2_1_as}\\
\dot{\bfv}_l &= \bfK(\bfg^p_l - \bfp_l) -\bfD\bfv_l \label{eq:dmp_left2_2_as}
\end{align}
\normalsize
\end{subequations}
In order to prove the stability of \eqref{eq:dmp_right2_1_as}--\eqref{eq:dmp_left2_2_as}, we consider the candidate Lyapunov function:
\begin{equation}
\small
\begin{split}
V^p(\bfx^p) &= \frac{1}{2}(\bfg^p_r-\bfp_r)\tr\bfK(\bfg^p_r-\bfp_r) + \frac{1}{2}\bfv_r\tr\bfv_r\\
    &\quad +\frac{1}{2}(\bfg^p_l-\bfp_l)\tr\bfK(\bfg^p_l-\bfp_l) + \frac{1}{2}\bfv_l\tr\bfv_l,\label{eq:lyapunov_fun_2_pos}
\end{split}
\normalsize
\end{equation}
where the state is defined as $\bfx^p = [\bfp_r\tr,\, \bfp_l\tr,\, \bfv_r\tr,\, \bfv_l\tr]\tr\in\mathbb{R}^{12}$.  The candidate Lyapunov function in \eqref{eq:lyapunov_fun_2_pos} is positive definite if $\bfK$ is a positive definite matrix, and it vanishes only at the equilibrium point $\hat{\bfx}^p =[{\bfg^{p}_{r}}\tr,\, {\bfg^{p}_{l}}\tr,\, \bfzero\tr,\, \bfzero\tr]\tr$ if and only if $\bfg^{p}_{r}-\bfg^{p}_{l} = \bfg^{p}_{rel}$. %To show that $V^p(\bfx^p)$ is a proper Lyapunov function, which implies that the system \eqref{eq:dmp_right1_as}--\eqref{eq:dmp_left2_as} is asymptotically stable and converges to $\hat{\bfx}^p$, we have to prove that $\dot{V}^p(\bfx^p)<0$ for each state $\bfx^p\neq\hat{\bfx}^p$ and that $\dot{V}^p(\bfx^p)=0$ at $\hat{\bfx}^p$. 
The time derivative of $V^p(\bfx^p)$ in \eqref{eq:lyapunov_fun_2_pos} can be written as:
\begin{equation*}
\small
\begin{split}
\dot{V}^p(\bfx^p) &= -\left[\cancel{\bfv_r} + \bfK_f(\bfg_{rel}-\bfp_{r,l})\right]\tr\bfK(\bfg^p_r-\bfp_r) \\
& -\left[\cancel{\bfv_l} - \bfK_f(\bfg_{rel}-\bfp_{r,l})\right]\tr\bfK(\bfg^p_l-\bfp_l) \\
&+ \cancel{\bfv_r\tr\bfK(\bfg^p_r-\bfp_r)} -\bfv_r\tr\bfD\bfv_r + \cancel{\bfv_l\tr\bfK(\bfg^p_l-\bfp_l)} -\bfv_l\tr\bfD\bfv_l
\end{split}
\normalsize
\end{equation*}
Recalling that $\bfg^{p}_{rel} = \bfg^{p}_{r}-\bfg^{p}_{l}$ and $\bfp_{r,l} = \bfp_r-\bfp_l$, after some algebraic operations we obtain:
\begin{equation*}
\small
\dot{V}^p(\bfx^p) = -\bfv_r\tr\bfD\bfv_r -\bfv_l\tr\bfD\bfv_l -(\bfg_{rel}-\bfp_{r,l})\tr\bfK_f\tr\bfK(\bfg_{rel}-\bfp_{r,l}) \normalsize
\end{equation*}
that is negative definite if $\bfK_f\tr\bfK$ is a positive definite matrix. The positive definitess of $\bfK_f\tr\bfK$ holds, for instance, if $\bfK_f$ and $\bfK$ are both diagonal and positive definite matrices. Note that $\dot{V}^p(\bfx^p)=0$ if and only if $\bfv_r = \bfv_l = \bfzero$ and $\bfg^{p}_{r}-\bfg^{p}_{l} = \bfp_r-\bfp_l$. The LaSalle's invariance theorem \cite{Slotine91} allows to conclude the stability of the system \eqref{eq:dmp_right2_1_as}--\eqref{eq:dmp_left2_2_as} and, as a consequence, the stability of the position part of C-DMPs. 

As for the position, the stability of the orientation part of C-DMPs, i.e. the stability of the system \eqref{eq:dmp_ori_right1}--\eqref{eq:dmp_ori_relative2} with coupling forces \eqref{eq:synchro_force_2_2} and \eqref{eq:synchro_force_2_3}, can be proved considering the asymptotic behavior of \eqref{eq:dmp_ori_right1}--\eqref{eq:dmp_ori_relative2}. As discussed in Case I, the relative DMP in \eqref{eq:dmp_ori_relative1} and \eqref{eq:dmp_ori_relative2} is decoupled from the other equations and it is asymptotically stable ($\bfq_{rel}\rightarrow\bfg_{rel}^q$ and $\bfomega_{rel}\rightarrow\bfzero$). Given this, we can rewrite the asymptotic behavior of \eqref{eq:dmp_ori_right1}--\eqref{eq:dmp_ori_left2} as:
\begin{subequations}
\small
\begin{align}
\dot{\bfq}_r &= \frac{1}{2}\left(\tilde{\bfomega}_r + [0,\, (\bfK_f{\bfe_{r,l}})\tr]\tr\right) \ast \bfq_r  \label{eq:dmp_ori_right2_1_as}\\
\dot{\bfomega}_r &= \bfK\bfe_{r} -\bfD\bfomega_r
\label{eq:dmp_ori_right2_2_as}\\
\dot{\bfq}_l &= \frac{1}{2}\left(\tilde{\bfomega}_l + [0,\, (\bfK_f{\bfe_{l,r}})\tr]\tr\right) \ast \bfq_l \label{eq:dmp_ori_left2_1_as}\\
\dot{\bfomega}_l &= \bfK\bfe_{l} -\bfD\bfomega_l
\label{eq:dmp_ori_left2_2_as}
\end{align}
\normalsize
\end{subequations}
where we put $\bfe_{r} = 2\text{vec}(\bfg^q_r \ast \overline{\bfq}_r)$, $\bfe_{l} = 2\text{vec}(\bfg^q_l \ast \overline{\bfq}_l)$, $\bfe_{r,l} = 2 \text{vec}{(\bfg^{q}_{rel} \ast (\overline{\bfq_r\ast\overline{\bfq}_l}) )}$, and $\bfe_{l,r} = -\bfq_{l,r}\ast\bfe_{r,l}\ast\overline{\bfq}_{l,r}$ .

In order to prove the stability of \eqref{eq:dmp_ori_right2_1_as}--\eqref{eq:dmp_ori_left2_2_as}, we consider the candidate Lyapunov function:
\begin{equation}
\small
\begin{split}
V^{q}(\bfx^q) &= V_e(\bfg^{q}_{r},\bfq_r) + \frac{1}{4}\bfomega_{r}\tr\bfK^{-1}\bfomega_{r} + V_e(\bfg^{q}_{l},\bfq_l) + \frac{1}{4}\bfomega_{l}\tr\bfK^{-1}\bfomega_{l}\\
&\quad+V_e(\bfg^{q}_{rel},\bfq_r\ast\overline{\bfq}_l)
\label{eq:lyapunov_fun_ori2}
\end{split}
\normalsize
\end{equation}
where $V_e(\bfq_1,\bfq_2)=\left(\eta_1 - \eta_{2}\right)^2 + \Vert\bfepsilon_1-\bfepsilon_2\Vert^2$ is defined as in \eqref{eq:lyapunov_fun_rel_ori} and the state $\bfx^q = [\bfq_{r}\tr,\,\bfq_{l}\tr,\,\bfomega_{r}\tr,\,\bfomega_{l}\tr]\tr$. The candidate Lyapunov function in \eqref{eq:lyapunov_fun_rel_ori} is positive definite and it vanishes only at the equilibrium $\hat{\bfx}^{q} = [{\bfg^{q}_{r}}\tr,\,{\bfg^{q}_{l}}\tr,\,\bfzero\tr,\,\bfzero\tr]\tr$ if and only if $\bfg^{q}_{rel} = \bfg^{q}_{r}\ast\overline{\bfg}^{q}_l$. The time derivative of $V^q(\bfx^q)$ can be written as:
\begin{equation}
\small
\begin{split}
\dot{V}^{q}(\bfx^q) &= \dot{V}_e(\bfg^{q}_{r},\bfq_r) + \dot{V}_e(\bfg^{q}_{l},\bfq_l)\\
&\quad+ \frac{1}{2}\bfomega_{r}\tr\bfK^{-1}[\bfK\bfe_r -\bfD\bfomega_r  + \bfK_f \bfe_{rel} - \bfD_f\bfomega_e]\\
              &\quad+ \frac{1}{2}\bfomega_{l}\tr\bfK^{-1}[\bfK\bfe_l -\bfD\bfomega_l - \bfK_f \bfe_{rel} + \bfD_f\bfomega_e]\\
              &\quad+\dot{V}_e(\bfg^{q}_{rel},\bfq_r\ast\overline{\bfq}_l)
\label{eq:dot_lyapunov_fun_ori2}
\end{split}
\normalsize
\end{equation}
where we used the definitions of $\dot{\bfomega}_{r}$ and $\dot{\bfomega}_{l}$ in \eqref{eq:dmp_ori_right2_2_as} and \eqref{eq:dmp_ori_left2_2_as} respectively. %Following similar steps as in \eqref{eq:V_dot_ori_rel} and 
Considering the expression of $\dot{V}_e$ in \eqref{eq:Ve_dot}, and recalling that $\bfomega_e=\bfomega_r-\bfomega_l$ is the angular velocity associated to the quaternion $\bfq_r\ast\overline{\bfq}_l$, it is possible to rewrite \eqref{eq:dot_lyapunov_fun_ori2} as:
\begin{equation}
\small
\begin{split}
\dot{V}^{q}(\bfx^q) &= -\frac{1}{2}\bfomega_{r}\tr\bfD_k\bfomega_{r} -\frac{1}{2}\bfomega_{l}\tr\bfD_k\bfomega_{l} -\frac{1}{2}\bfomega_{e}\tr\bfK^{-1}\bfD_f\bfomega_{e}\\
&\quad + \bfomega_{e}\tr\left(\bfK^{-1}\bfK_f \bfe_{rel} - \text{vec}(\bfg^{q}_{rel}\ast\left(\overline{\bfq_r\ast\overline{\bfq}_l}\right)\right)
\label{eq:dot_lyapunov_fun_ori2_2}
\end{split}
\normalsize
\end{equation}
By choosing  $\bfK_f = \bfK$ 
the derivative of the Lyapunov function becomes
\begin{equation*}
\small
\begin{split}
\dot{V}^{q}(\bfx^q) = -\bfomega_{r}\tr\bfD\bfomega_{r} -\bfomega_{l}\tr\bfD\bfomega_{l} -\bfomega_{e}\tr\bfD_f\bfomega_{e} \leq 0
\end{split}
\normalsize
\end{equation*}
The derivative of the Lyapunov function is negative semidefinite and it vanishes if and only if $\bfomega_{r} = \bfomega_{l} = \bfzero$. The LaSalle's invariance theorem \cite{Slotine91} allows to conclude the stability of the system \eqref{eq:dmp_ori_right2_1_as}--\eqref{eq:dmp_ori_left2_2_as} and, as a consequence, the stability of the orientation part of C-DMPs.

The conducted stability analysis \textcolor{red}{tells N things ... Say about relative goal, K and D diagonal, $K_f = K$}

Given the orientation stiffness gains $\bfK = k\bfI$, the orientation damping gains $\bfD = d\bfI$ are chosen as $\bfD = \sqrt{4k}\bfI$ to have a critically damped system \cite{Weitschat16}.

The original DMPs contain a constant scaling term ($\tau > 0$) used to speed-up or slow-down the motion execution \cite{DMP}. The scaling term can be eventually added to the C-DMPs without compromising the stability

==> sections/Stability_proof/Case3.tex <==
\subsection*{Case III} In this case, coupling forces are defined as:
\begin{subequations}
\small
\begin{align}
\bff^p_{r,l} &= \bfK_f(\bfp_{rel} - \bfp_{r,l}), ~\bff^p_{l,r} = -\bff^p_{r,l}, \label{eq:synchro_force_3_1}\\
\bff^v_{r,l} &=  \bfD_f(\bfv_{rel} - \bfv_{r,l}), ~\bff^v_{l,r} = -\bff^v_{r,l},\label{eq:synchro_force_3_2}\\
\bff^q_{r,l} &= \bfK_f 2 \text{vec}{(\bfq_{rel} \ast \overline{\bfq}_{r,l} )}, ~\bff^{q}_{l,r} = -\bfq_{l,r}\ast\bff^{q}_{r,l}\ast\overline{\bfq}_{l,r},\label{eq:synchro_force_3_3}\\
\bff^{\omega}_{r,l} &=  \bfD_f(\bfomega_{rel} - \bfomega_{r,l}), ~\bff^{\omega}_{l,r} = -\bfq_{l,r}\ast\bff^{\omega}_{r,l}\ast\overline{\bfq}_{l,r}. \label{eq:synchro_force_3_4}
\end{align}
\normalsize
\end{subequations}

Let us first focus on the position, i.e. on the stability of the system of differential equations \eqref{eq:dmp_right1}--\eqref{eq:dmp_relative2} with coupling forces defined as in \eqref{eq:synchro_force_3_1}--\eqref{eq:synchro_force_3_2}. As discussed in Case I, the relative DMP is stable ($\bfp_{rel}\rightarrow\bfg^{p}_{rel}$ and $\bfv_{rel}\rightarrow\bfzero$) if the gain matrices $\bfK$ and $\bfD$ are positive definite, and we can conclude the stability of C-DMPs by analyzing the asymptotic behavior of \eqref{eq:dmp_right1}--\eqref{eq:dmp_left2}. For $t\rightarrow+\infty$, we can rewrite \eqref{eq:dmp_right1}--\eqref{eq:dmp_left2} as:
\begin{subequations}
\small
\begin{align}
\dot{\bfp}_r &= \bfv_r + \bfK_f(\bfg_{rel} - \bfp_{r,l}) \label{eq:dmp_right3_1_as}\\
\dot{\bfv}_r &= \bfK(\bfg^p_r - \bfp_r)-\bfD\bfv_r - \bfD_f \bfv_{r,l} \label{eq:dmp_right3_2_as}\\
\dot{\bfp}_l &= \bfv_l - \bfK_f(\bfg_{rel} - \bfp_{r,l}) \label{eq:dmp_left3_1_as}\\
\dot{\bfv}_l &= \bfK(\bfg^p_l - \bfp_l) -\bfD\bfv_l + \bfD_f\bfv_{r,l}\label{eq:dmp_left3_2_as}
\end{align}
\normalsize
\end{subequations}
We consider the candidate Lyapunov function:
\begin{equation}
\small
\begin{split}
V^p(\bfx^p) &= \frac{1}{2}(\bfg^p_r-\bfp_r)\tr\bfK(\bfg^p_r-\bfp_r) + \frac{1}{2}\bfv_r\tr\bfv_r\\
    &\quad +\frac{1}{2}(\bfg^p_l-\bfp_l)\tr\bfK(\bfg^p_l-\bfp_l) + \frac{1}{2}\bfv_l\tr\bfv_l,\label{eq:lyapunov_fun_3_pos}
\end{split}
\normalsize
\end{equation}
where the state is defined as $\bfx^p = [\bfp_r\tr,\, \bfp_l\tr,\, \bfv_r\tr,\, \bfv_l\tr]\tr\in\mathbb{R}^{12}$.  The candidate Lyapunov function in \eqref{eq:lyapunov_fun_3_pos} is positive definite if $\bfK$ is a positive definite matrix, and it vanishes only at the equilibrium point $\hat{\bfx}^p =[{\bfg^{p}_{r}}\tr,\, {\bfg^{p}_{l}}\tr,\, \bfzero\tr,\, \bfzero\tr]\tr$ if and only if $\bfg^{p}_{r}-\bfg^{p}_{l} = \bfg^{p}_{rel}$. %To show that $V^p(\bfx^p)$ is a proper Lyapunov function, which implies that the system \eqref{eq:dmp_right3_1_as}--\eqref{eq:dmp_left3_2_as} is asymptotically stable and converges to $\hat{\bfx}^p$, we have to prove that $\dot{V}^p(\bfx^p)<0$ for each state $\bfx^p\neq\hat{\bfx}^p$ and that $\dot{V}^p(\bfx^p)=0$ at $\hat{\bfx}^p$. 
The time derivative of $V^p(\bfx^p)$ in \eqref{eq:lyapunov_fun_3_pos}  can be written as:
\begin{equation*}
\small
\begin{split}
\dot{V}^p(\bfx^p) &= -\left[\cancel{\bfv_r} + \bfK_f(\bfg_{rel}-\bfp_{r,l})\right]\tr\bfK(\bfg^p_r-\bfp_r) -\bfv_r\tr\bfD\bfv_r\\
& -\left[\cancel{\bfv_l} - \bfK_f(\bfg_{rel}-\bfp_{r,l})\right]\tr\bfK(\bfg^p_l-\bfp_l) -\bfv_l\tr\bfD\bfv_l\\
&+ \cancel{\bfv_r\tr\bfK(\bfg^p_r-\bfp_r)}  + \cancel{\bfv_l\tr\bfK(\bfg^p_l-\bfp_l)} -\bfv_{r,l}\tr\bfD_f\bfv_{r,l}
\end{split}
\normalsize
\end{equation*}
Recalling that $\bfg^{p}_{rel} = \bfg^{p}_{r}-\bfg^{p}_{l}$ and $\bfp_{r,l} = \bfp_r-\bfp_l$, after some algebraic operations we obtain:
\begin{equation*}
\small
\begin{split}
\dot{V}^p(\bfx^p) &= -\bfv_r\tr\bfD\bfv_r -\bfv_l\tr\bfD\bfv_l -\bfv_{r,l}\tr\bfD_f\bfv_{r,l}\\ &\quad-(\bfg_{rel}-\bfp_{r,l})\tr\bfK_f\tr\bfK(\bfg_{rel}-\bfp_{r,l}) 
\end{split}
\normalsize
\end{equation*}
that is negative definite if $\bfK_f\tr\bfK$ is a positive definite matrix. The positive definitess of $\bfK_f\tr\bfK$ holds, for instance, if $\bfK_f$ and $\bfK$ are both diagonal and positive definite matrices. Note that $\dot{V}^p(\bfx^p)=0$ if and only if $\bfv_r = \bfv_l = \bfzero$ and $\bfg^{p}_{r}-\bfg^{p}_{l} = \bfp_r-\bfp_l$. The LaSalle's invariance theorem \cite{Slotine91} allows to conclude the stability of the system \eqref{eq:dmp_right1_as}--\eqref{eq:dmp_left2_as} and, as a consequence, the stability of the position part of C-DMPs. 
